DeepTreeGANv2: Iterative Pooling of Point Clouds

In High Energy Physics, detailed and time-consuming simulations are used for particle interactions with detectors. To bypass these simulations with a generative model, the generation of large point clouds in a short time is required, while the complex dependencies between the particles must be correctly modelled. Particle showers are inherently tree-based processes, as each particle is produced by the decay or detector interaction of a particle of the previous generation. In this work, we present a significant extension to DeepTreeGAN, featuring a critic, that is able to aggregate such point clouds iteratively in a tree-based manner. We show that this model can reproduce complex distributions, and we evaluate its performance on the public JetNet 150 dataset.

==> Makefile <==
TEX = 'lualatex'
JOBDIR = 'build'
NAME = 'DeepTreeGAN'

paper: paper.tex
	[ -d $(JOBDIR) ] || mkdir build
	$(TEX) -jobname=$(JOBDIR)/$(NAME) --file-line-error --halt-on-error  --shell-escape "\input{paper.tex}"

all: paper


